Big Data-driven Automated Anomaly Detection and Performance Forecasting in Mobile Networks

The massive amount of data available in operational mobile networks offers an invaluable opportunity for operators to detect and analyze possible anomalies and predict network performance. In particular, application of advanced machine learning (ML) techniques on data aggregated from multiple sources can lead to important insights, not only for the detection of anomalous behavior but also for performance forecasting, thereby complementing classic network operation and maintenance solutions with intelligent monitoring tools. In this paper, we propose a novel framework that aggregates diverse data sets (e.g. configuration, performance, inventory, locations, user speeds) from an operational LTE network and applies ML algorithms to diagnose network issues and analyze their impact on key performance indicators. To this end, pattern identification and time-series forecasting algorithms are used on the ingested data. Results show that proposed framework can indeed be leveraged to automate the identification of anomalous behaviors associated with the spatial-temporal characteristics, and predict customer impact in an accurate manner.

==> notes.tex <==
\begin{figure}[t!]
\centering
 \includegraphics[trim={0.25cm 0.25cm 0.25cm 0.25cm},scale=0.29,clip]{figures/ts_region3greyv1}  
   \caption{KPI signatures representing normal behaviours (average speed $> 50$ Km/h).}
\label{fig2}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[trim={0.25cm 0.25cm 0.25cm 0.25cm},scale=0.29,clip]{figures/ts_region5greyv1} 
\caption{KPI signatures representing abnormal behaviours (average speed $> 50$ Km/h).}
\label{fig3}
\end{figure}
\begin{figure}[t]
\centering
 \includegraphics[width=\columnwidth]{figures/bagging_predicted_vs_true_region5v3.png}%predicted_vs_true_normal}  
   \caption{Predicted, last, and real KPI value. Time series with abnormal behaviours.}
\label{fig4a}
\end{figure}
